Multiscale modeling of kinetic sluggishness in equiatomic NiCoCr and NiCoCrFeMn single-phase solid solutions

Complex, concentrated, multi-component alloys have been shown to display outstanding thermo-mechanical properties, that have been typically attributed to sluggish diffusion, entropic, and lattice distortion effects. Here, we investigate two metal alloys with such exemplary properties, the equiatomic, single-phase, face-centered-cubic (FCC) alloys NiCoCr and NiCoCrFeMn, and we compare their microstructural kinetics to the behaviors in a pure-Ni FCC metal. We perform long-time, kinetic Monte Carlo (kMC) simulations, and we analyze in detail the kinetics of atomic vacancies. We find that vacancies in both concentrated alloys exhibit subdiffusive thermally driven dynamics, in direct contrast to the diffusive dynamics of pure Ni. Subdiffusive dynamics shall be attributed to dynamical sluggishness, that is modeled by a fractional Brownian random walk. Furthermore, we analyze the statistics of waiting times, and we interpret long power-law-distributed rest periods as a direct consequence of barriers' energy-scales and lattice distortions.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
